Characterization and Performance of PADME's Cherenkov-Based Small-Angle Calorimeter

The PADME experiment, at the Laboratori Nazionali di Frascati (LNF), in Italy, will search for invisible decays of the hypothetical dark photon via the process $e^+e^-\rightarrow \gamma A'$, where the $A'$ escapes detection. The dark photon mass range sensitivity in a first phase will be 1 to 24 MeV. We report here on measurement and simulation studies of the performance of the Small-Angle Calorimeter, a component of PADME's detector dedicated to rejecting 2- and 3-gamma backgrounds. The crucial requirement is a timing resolution of less than 200 ps, which is satisfied by the choice of PbF$_2$ crystals and the newly released Hamamatsu R13478UV photomultiplier tubes (PMTs). We find a timing resolution of 81 ps (with double-peak separation resolution of 1.8 ns) and a single-crystal energy resolution of 5.7%/$\sqrt{E}$ with light yield of 2.07 photo-electrons per MeV, using 100 to 400 MeV electrons at the Beam Test Facility of LNF. We also propose the investigation of a two-PMT solution coupled to a single PbF$_2$ crystal for higher-energy applications, which has potentially attractive features.

==> preamble.tex <==
% BEGIN Custom packages

\usepackage{subcaption} % subfigure env. has to come before hyperref

\usepackage{balance}
\usepackage{lastpage}
% \usepackage{lastpage}
% \makeatletter
%     \def\balanceissued{unbalanced}%flag to indicate if \balance has been used
%     \let\oldbibitem\bibitem
%     \def\bibitem{%
%         \ifnum\thepage=\lastpage@lastpage%
%             \expandafter\ifx\expandafter\relax\balanceissued\relax\else%
%                 \balance%
%                 \gdef\balanceissued{\relax}\fi%
%             \else\fi%
%         \oldbibitem}
% \makeatother

\usepackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
%,pagecolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\RequirePackage{doi}

%% The graphicx package provides the includegraphics command.
\usepackage{graphicx}
%% The amssymb package provides various useful mathematical symbols
\usepackage{amssymb}
%% The amsthm package provides extended theorem environments
%% \usepackage{amsthm}

%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers after \end{frontmatter}.
\usepackage{lineno}

\usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}
% activate={true,nocompatibility} - activate protrusion and expansion
% final - enable microtype; use "draft" to disable
% tracking=true, kerning=true, spacing=true - activate these techniques
% factor=1100 - add 10% to the protrusion amount (default is 1000)
% stretch=10, shrink=10 - reduce stretchability/shrinkability (default is 20/20)
\microtypecontext{spacing=nonfrench}

\usepackage{feynmp} % feynman diagrams
\DeclareGraphicsRule{*}{mps}{*}{}

\usepackage{textcomp} % for \textdegree macro
\usepackage[product-units = power, range-units = single, list-units = single]{siunitx}
% nice unit formatting
\DeclareSIUnit{\pe}{p.e.}
\usepackage{color} % text color
\usepackage{soul}
\usepackage[capitalize,nameinlink]{cleveref} % use \cref instead of \ref
\usepackage{todonotes} % missing figure place holder

% \usepackage[sorting=none,backend=biber]{biblatex}
% \addbibresource{bibliography.bib}

\usepackage[T1]{fontenc} % if needed
\usepackage[utf8]{inputenc}
% END Custom packages

% BEGIN Custom commands
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\pbfII}{PbF$_2$}
% END Custom commands


